Learning In Practice: Reasoning About Quantization

There is a mismatch between the standard theoretical analyses of statistical machine learning and how learning is used in practice. The foundational assumption supporting the theory is that we can represent features and models using real-valued parameters. In practice, however, we do not use real numbers at any point during training or deployment. Instead, we rely on discrete and finite quantizations of the reals, typically floating points. In this paper, we propose a framework for reasoning about learning under arbitrary quantizations. Using this formalization, we prove the convergence of quantization-aware versions of the Perceptron and Frank-Wolfe algorithms. Finally, we report the results of an extensive empirical study of the impact of quantization using a broad spectrum of datasets.

==> farm-gisette-results.tex <==

\begin{table}
  \centering
  \footnotesize
  \caption{Test set accuracies on the gisette dataset (left) and the farm-ads dataset (right) for different quantizations. For floating points, each row represents a different value of the exponent part. One bit in the bit budget is assigned for the sign and the rest of the bits are used for the mantissa.  Green cells are closer to the maximum possible accuracy, while redder cells are closer to the majority baseline.}   
  \begin{tabular}{r|cccc}
    \multicolumn{5}{c}{Results on gisette dataset} \\
    \toprule

                 & \multicolumn{4}{c}{Bit budget for fixed points}       \\
    Range        & 6 bits      & 7 bits      & 8 bits      & 9 bits      \\
    \midrule
    $[-8,8]$     & \cc{90}{50} & \cc{89}{50} & \cc{62}{50} & \cc{50}{50} \\ 
    $[-16,16]$   & \cc{92}{50} & \cc{93}{50} & \cc{88}{50} & \cc{88}{50} \\ 
    $[-32,32]$   & \cc{50}{50} & \cc{90}{50} & \cc{94}{50} & \cc{93}{50} \\ 
    $[-64,64]$   & \cc{50}{50} & \cc{50}{50} & \cc{91}{50} & \cc{94}{50} \\ 
    $[-128,128]$ & \cc{50}{50} & \cc{50}{50} & \cc{50}{50} & \cc{89}{50} \\ 
    \bottomrule
  % \end{tabular}\hfill
  % \begin{tabular}{r|cccc}
  %   \toprule
    \# exponent  & \multicolumn{4}{c}{Bit budget for floating points}    \\
    bits         & 6 bits      & 7 bits      & 8 bits      & 9 bits      \\
    \midrule
    1            & \cc{57}{50} & \cc{71}{50} & \cc{82}{50} & \cc{82}{50} \\
    2            & \cc{88}{50} & \cc{81}{50} & \cc{88}{50} & \cc{82}{50} \\
    3            & \cc{81}{50} & \cc{85}{50} & \cc{83}{50} & \cc{94}{50} \\
    4            & \cc{50}{50} & \cc{51}{50} & \cc{88}{50} & \cc{94}{50} \\
    5            & --          & \cc{50}{50} & \cc{50}{50} & \cc{77}{50} \\
    6            & --          & --          & \cc{50}{50} & \cc{50}{50} \\
    7            & --          & --          & --          & \cc{50}{50} \\
    \bottomrule
  \end{tabular}\hfill
  \begin{tabular}{r|cccc}
    \multicolumn{5}{c}{Results on farm-ads dataset} \\    
    \toprule
                 & \multicolumn{4}{c}{Bit budget for fixed points}       \\
    Range        & 9 bits      & 10 bits     & 11 bits     & 12 bits     \\
    \midrule
    $[-8,8]$     & \cc{83}{51} & \cc{82}{51} & \cc{79}{51} & \cc{86}{51} \\ 
    $[-16,16]$   & \cc{77}{51} & \cc{77}{51} & \cc{76}{51} & \cc{87}{51} \\ 
    $[-32,32]$   & \cc{51}{51} & \cc{59}{51} & \cc{66}{51} & \cc{88}{51} \\ 
    $[-64,64]$   & \cc{51}{51} & \cc{51}{51} & \cc{56}{51} & \cc{87}{51} \\ 
    $[-128,128]$ & \cc{51}{51} & \cc{51}{51} & \cc{52}{51} & \cc{88}{51} \\ 
    \bottomrule
  % \end{tabular}\hfill
  % \begin{tabular}{r|cccc}
  %   \toprule    
    \# exponent  & \multicolumn{4}{c}{Bit budget for floating points}    \\
    bits         & 7 bits      & 8 bits      & 9 bits      & 10 bits     \\
    \midrule
    1            & \cc{84}{51} & \cc{84}{51} & \cc{84}{51} & \cc{84}{51} \\
    2            & \cc{86}{51} & \cc{89}{51} & \cc{87}{51} & \cc{87}{51} \\
    3            & \cc{87}{51} & \cc{86}{51} & \cc{86}{51} & \cc{86}{51} \\
    4            & \cc{85}{51} & \cc{87}{51} & \cc{89}{51} & \cc{89}{51} \\
    5            & \cc{85}{51} & \cc{85}{51} & \cc{89}{51} & \cc{87}{51} \\
    6            & --          & \cc{85}{51} & \cc{85}{51} & \cc{85}{51} \\
    7            & --          & --          & --          & \cc{85}{51} \\
    \bottomrule
  \end{tabular}

  
  \label{tab:farm-gisette-results}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "nips_2018"
%%% End:


==> lemma-1-proof.tex <==
\section{Proof of Lemma 1}
\label{sec:proof-lemma-1}



% \jeff{WaiMing:  Can you remove the assumption that $d$ is a constant?  I don't think its needed, but I don't see the path to a simple proof that removes it.  This is common in CG, so not too worried about it.}

Without loss of generality, let the side length of the cube $M$ be $1$, so the side length of each quantization region $Q_a$ is $1/m^{1/d}$. Then, the diameter of each $Q_a$ is $\sqrt{d}/m^{1/d}$.

Now, consider a linear separator $F$ which is a $(d-1)$-dimensional subspace.
% Let it be spanned by $d-1$ orthogonal vectors $\{u_1, u_2, \ldots, u_{d-1}\}$.
Use any orthogonal basis spanning $F$ to define a $(d-1)$-dimensional grid within $F$. Place a set of $\Omega((m^{1/d})^{d-1}) = \Omega(m^{1-1/d})$ grid points on $F$ so that, along each axis of the basis, they are a distance of $\sqrt{d}/m^{1/d}$ apart. %\vs{Todo: Explain why it is possible to place such a grid.}
No two of these grid points can be in the same $Q_a$ because their separation is at least the diameter of a cell.  Thus, at least $\Omega(m^{1-1/d})$ quantization cells of $A$ must intersect the linear separator.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "supplementary"
%%% End:

